Tuning the Magnetic Properties of the CrMnFeCoNi Cantor Alloy

Magnetic properties of more than twenty Cantor alloy samples of varying composition were investigated over a temperature range of 5 K to 300 K and in fields of up to 70 kOe using magnetometry and muon spin relaxation. Two transitions are identified: a spin-glass-like transition that appears between 55 K and 190 K depending on composition, and a ferrimagnetic transition that occurs at approximately 43 K in multiple samples with widely varying compositions. The magnetic signatures at 43 K are remarkably insensitive to chemical composition. A modified Curie-Weiss model was used to fit the susceptibility data and to extract the net effective magnetic moment for each sample. The resulting values for the net effective moment were either diminished with increasing Cr or Mn concentrations or enhanced with decreasing Fe, Co, or Ni concentrations. Beyond a sufficiently large effective moment, the magnetic ground state transitions from ferrimagnetism to ferromagnetism. The effective magnetic moments, together with the corresponding compositions, are used in a global linear regression analysis to extract element-specific effective magnetic moments, which are compared to the values obtained by ab-initio based density functional theory (DFT) calculations. These moments provide the information necessary to controllably tune the magnetic properties of Cantor alloy variants.

==> extras/remove_bars <==
% Remove double bars from the document.
% Since there is no abstract in the supplementary material,
% we can get rid of the lines that normally appear around abstract.

\makeatletter
\renewcommand{\MaketitleBox}{%
  \resetTitleCounters
  \def\baselinestretch{1}%
  \begin{center}
    \def\baselinestretch{1}%
    \Large \@title \par
    \vskip 18pt
    \normalsize\elsauthors \par
    \vskip 10pt
    \footnotesize \itshape \elsaddress \par
  \end{center}
  \vskip 12pt
}
\makeatother
